TransDrift: Modeling Word-Embedding Drift using Transformer

In modern NLP applications, word embeddings are a crucial backbone that can be readily shared across a number of tasks. However as the text distributions change and word semantics evolve over time, the downstream applications using the embeddings can suffer if the word representations do not conform to the data drift. Thus, maintaining word embeddings to be consistent with the underlying data distribution is a key problem. In this work, we tackle this problem and propose TransDrift, a transformer-based prediction model for word embeddings. Leveraging the flexibility of transformer, our model accurately learns the dynamics of the embedding drift and predicts the future embedding. In experiments, we compare with existing methods and show that our model makes significantly more accurate predictions of the word embedding than the baselines. Crucially, by applying the predicted embeddings as a backbone for downstream classification tasks, we show that our embeddings lead to superior performance compared to the previous methods.

==> experiment_details.tex <==
We evaluate our models on a synthetic dataset, Yelp
Academic dataset (Crawford, 2018) and Amazon
Customer Review dataset (McAuley, 2018). For
each dataset, we consider 1000 drift instances with
each instance consisting of D1, D2, and Dsmall
2 during training. Here, the subscript 1 denotes the
source time-step t = 1 and subscript 2 denotes
the next time-step (i.e. t = 2) in which the underly-
ing text distribution has undergone a shift. Out of
these 1000 instances, we use 800 for training, 100
for validation, and the rest for testing.

\textbf{MLP}

\begin{itemize}
\item Model parameters = 20250
\end{itemize}
\begin{itemize}
\item Max-epochs = 50, model-dim = 50, warmup = 30, LR = 5e-4, Batch size = 100
\end{itemize}

\section{Synthetic Dataset}

\begin{itemize}
\item Vocab size for :-
\begin{enumerate}
\item D1 = 100,
\item D2 = 100,
\item D2-small-50 = 50,
\item D2-small-30 = 30,
\item D2-small-20 = 20

\end{enumerate}
\end{itemize}
\begin{itemize}
\item Dimension for D1, D2, D2-small-s and predicted embedding is 50.
\end{itemize}


\textbf{TransDrift}

\begin{itemize}
\item Model parameters - 504250
\end{itemize}
\begin{itemize}
\item Max-epochs = 100, num-heads = 1, model-dim = 100, num-layers = 4, LR = 5e-4, Batch size = 100
\end{itemize}

\section{Yelp Dataset}


\begin{itemize}
\item Vocab size for :-
\begin{enumerate}
\item D1 = 1727,
\item D2 = 1727,
\item D2-small-50 = 1396,
\item D2-small-30 = 901,
\item D2-small-20 = 634
\end{enumerate}
\end{itemize}
            
\begin{itemize}
\item Dimension for D1, D2, D2-small-s and predicted embedding is 50.
\end{itemize}
 
 \textbf{TransDrift}
Ran on CPU.
\begin{itemize}
\item Model parameters - 1833650
\end{itemize}

\begin{itemize}
\item Using word2vec, Max-epochs = 100, num-heads = 4, model-dim = 192, num-layers = 4, LR = 5e-4, Batch size = 100
\end{itemize}


\section{Amazon Customer Review Dataset}

\begin{itemize}
\item  Vocab size for :-
\begin{enumerate}
\item D1 = 5018,
\item D2 = 5018,
\item D2-small-50 = 3323,
\item D2-small-30 = 2235,
\item D2-small-20 = 1603
\end{enumerate}
\end{itemize}
    
\begin{itemize}
\item Dimension for D1, D2, D2-small-s and predicted embedding is 50.
\end{itemize}


\textbf{TransDrift}
Ran on CPU.
\begin{itemize}
\item Model paramters - 1833650
\end{itemize}
\begin{itemize}
\item Using word2vec, Max-epochs = 100, num-heads = 4, model-dim = 192, warmup = 30, num-layers = 4, LR = 5e-4, Batch size = 100
\end{itemize}


\section{Downstream}
\begin{itemize}
\item E1 and E2_small_30 is used to predict the embeddings using transformer. These predicted embeddings are used in the downstream tasks.
\end{itemize}
 
\subsection{Synthetic Dataset}
Not done

\subsection{Yelp Dataset}

Multi-label star classification

\begin{itemize}
\item 20k reviews : 10k from each time stamp t1 and t2
\item 8:2 train-test split, epochs = 100, batch-size = 64
\end{itemize}



% Model Summary

Model: "model"                                                                                                               
\begin{table}[]
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Layer (type)} & \textbf{Output Shape} & \textbf{Param \#} \\ \midrule
input\_1 (InputLayer) & (None, 150)           & 0                 \\
embedding (Embedding) & (None, 150, 50)       & 1611750           \\
lstm (LSTM)           & (None, 128)           & 91648             \\
dense (Dense)         & (None, 5)             & 645               \\ \bottomrule
\end{tabular}
\end{table}

Total params: 1,704,043
Trainable params: 92,293
Non-trainable params: 1,611,750 


\subsection{Amazon Customer Review Dataset}


\begin{itemize}
\item Number of reviews :-
\begin{enumerate}
\item  Electronics - 5682
\item Kitchen - 5946
\item DVD - 3587
\end{enumerate}
\end{itemize}

\begin{itemize}
\item 8:2 train-test split, epochs = 100, batch-size = 64
\end{itemize}

%Model summary

Model: "model"               

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Layer (type)} & \textbf{Output Shape} & \textbf{Param \#} \\ \midrule
input\_1 (InputLayer) & (None, 150)           & 0                 \\
embedding (Embedding) & (None, 150, 50)       & 747250            \\
lstm (LSTM)           & (None, 150, 128)      & 91648             \\
dropout (Dropout)     & (None, 150, 128)      & 0                 \\
lstm\_1 (LSTM)        & (None, 150, 128)      & 131584            \\
dropout\_1 (Dropout)  & (None, 150, 128)      & 0                 \\
lstm\_2 (LSTM)        & (None, 128)           & 131584            \\
dense (Dense)         & (None, 1)             & 129               \\ \bottomrule
\end{tabular}
\end{table}

Total params: 1,102,195
Trainable params: 354,945
Non-trainable params: 747,250

%%


Table 4: 
For amazon, we have reviews from D1 and D2 used in downstream. E2 is trained on D2, it is performing worse. 
For yelp, we have reviews from D2 in downstream. E2 is trained on D2, hence it is performing better. 
